Hydra: Resilient and Highly Available Remote Memory

We present Hydra, a low-latency, low-overhead, and highly available resilience mechanism for remote memory. Hydra can access erasure-coded remote memory within a single-digit microsecond read/write latency, significantly improving the performance-efficiency trade-off over the state-of-the-art -- it performs similar to in-memory replication with 1.6X lower memory overhead. We also propose CodingSets, a novel coding group placement algorithm for erasure-coded data, that provides load balancing while reducing the probability of data loss under correlated failures by an order of magnitude. With Hydra, even when only 50% of memory is local, unmodified memory-intensive applications achieve performance close to that of the fully in-memory case in the presence of remote failures and outperform the state-of-the-art solutions by up to 4.35X.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

%\paragraph{{\bf PM Backup}} \rev{Local PM backup can significantly improve the performance of DBMSs in a disaggregated cluster. 
%However, our experiments show that {\name} can almost match the performance of local PM backup -- {\name}'s application-level performance varies within 0.94--1.09$\times$ of that with PM backup.
%Moreover, replacing SSD with PM throughout the cluster may not always be feasible.}%\mosharaf{Given the many times we mention PM in eval now, we should consider bringing PM discussion earlier. Adding PM costs new money; leveraging existing DRAM is free.}
%\mosharaf{We can bring this into TCO savings analysis.}
%\rev{
%	While providing resiliency using unused remote DRAM is free, PM for backup costs about $11.13\$$/GB \cite{pm-price}.
%	Accounting for the additional PM cost, the savings of disaggregation over 3 years drops from $6.3$\% to $3.5$\% for Google's example (Table \ref{tab:cost}) if a standard machine leverages the remote memory up to the same size of local memory.
%}

\paragraph{{\bf Application with Vector Instructions.}} \rev{ {\name} relies on x86 AVX instructions for erasure coding that can run on commodity x86 hardware.
However, if applications also use vector instructions, {\name} may suffer from the interference between legacy code and AVX instructions as they share the same set of registers\cite{avx-interference}.
Recent NICs \cite{mlx-ec} often support 
%hardware offloading of 
erasure coding
%Programmable NICs can perform erasure coding and directly write to remote machines;
which can help offload {\name} data plane to NICs.}%\mosharaf{Did anyone ask this?}

\paragraph{{\bf DMA Isolation and Scalability}} \rev{In native RDMA, due to RNIC resource contention, performance drops when multiple applications run together or the number of reliable connections increases~\cite{frdma, fasst}. 
%For example, throughput of RDMA writes gets 10$\times$ worse when the number of connections grows from 10 to 200.
However, recent work~\cite{lite, justitia, scale-rpc} show that virtualization of RNIC resources can ensure native performance at scale.
New NIC designs are also proposed~\cite{onerma, fairnic} for native RDMA performance at scale in multi-tenant datacenters.
Integrating {\name} with these systems can ensure seamless performance even with 100s of reliable connections.}
